Discovery of an Inflated Hot Neptune and Its Formation from Jovian Mass Loss

The production of Neptune-like planets with orbital periods of 3--6 days is challenging for conventional models of high-eccentricity migration. We present the discovery and characterization of TOI-2195~A~b, an inflated hot Neptune ($P = 4.16$ days, $m_p= 1.46M_{\rm Nep},\,R_p = 0.79R_{\rm J}$) orbiting an early K-type star with a wide binary companion at $\sim 600$~au. Detection of the Rossiter-McLaughlin effect at $\sim2.6\sigma$ confidence with Magellan/PFS reveals the planet is likely on a near-polar orbit with a sky-projected stellar obliquity $\lambda = {109^{+35}_{-53}} ^{\circ}$. We perform coupled dynamical and structural modeling that reproduces the observed characteristics of the system. We show that the planet may have originated as a cold, Jovian planet that was excited to high eccentricities via the stellar Eccentric Kozai-Lidov (EKL) mechanism, where it lost up to $\sim90\%$ of its mass via Roche lobe overflow during close periastron passages, enabling rapid tidal migration and radius inflation due to tidal heating. TOI-2195 A b provides a test for planetary migration theories, and our simulations suggest that puffy hot Neptunes originated as more massive Jovians that underwent mass loss during high-eccentricity migration.

==> tables/rv_data.tex <==
% bjdtdb, rv, rverr, instrument
2459456.85033 & 38136 & 35 & CHIRON \\
2459463.80033 & 38017 & 61 & CHIRON \\
2459485.70333 & 38203 & 24 & CHIRON \\
2459496.66990 & 38191 & 56 & CHIRON \\
2459539.63641 & 38086 & 26 & CHIRON \\
2459542.63262 & 38135 & 35 & CHIRON \\
2459546.54836 & 38121 & 22 & CHIRON \\
2459898.62713 & 38123 & 24 & CHIRON \\
2459900.72591 & 38132 & 32 & CHIRON \\
2459902.64032 & 38129 & 23 & CHIRON \\
2460180.90120 & -6.9 & 3.1 & PFS \\
2460211.86336 & -2.6 & 2.5 & PFS \\
2460218.85096 & -14.2 & 3.6 & PFS \\
2460270.63162 & 14.8 & 2.7 & PFS \\
2460273.71735 & -9.4 & 2.8 & PFS \\
2460277.61871 & -10.7 & 3.0 & PFS \\
2460299.55808 & 2.9 & 2.6 & PFS \\
2460300.56438 & 2.8 & 2.8 & PFS \\
2460921.74019 & 0.0 & 2.6 & PFS \\
2460921.74734 & 7.0 & 2.6 & PFS \\
2460921.75470 & 2.5 & 2.4 & PFS \\
2460921.76194 & 0.9 & 2.5 & PFS \\
2460921.76905 & 1.7 & 2.2 & PFS \\
2460921.77641 & 1.0 & 2.4 & PFS \\
2460921.78363 & 2.1 & 2.3 & PFS \\
2460921.79080 & -7.7 & 2.2 & PFS \\
2460921.79808 & -1.4 & 2.3 & PFS \\
2460921.80523 & -9.5 & 2.1 & PFS \\
2460921.81263 & -1.9 & 2.0 & PFS \\
2460921.81984 & 2.7 & 2.1 & PFS \\
2460921.82708 & -3.5 & 2.1 & PFS \\
2460921.83412 & -6.7 & 2.3 & PFS \\
2460921.84149 & -4.1 & 2.4 & PFS \\
2460921.84882 & -6.4 & 2.4 & PFS \\
2460921.85599 & 5.5 & 2.4 & PFS \\
2460921.86330 & 10.7 & 2.6 & PFS \\
2460921.87056 & -1.4 & 2.4 & PFS \\
2460921.87760 & 6.6 & 2.6 & PFS \\
2460921.88503 & 1.0 & 2.4 & PFS \\
2460921.89228 & -2.7 & 2.5 & PFS \\
2460987.63255 & 5.6 & 3.0 & PFS \\
2460988.66909 & -2.1 & 2.9 & PFS \\
2460989.68632 & -11.0 & 2.3 & PFS \\
2460990.64506 & 8.8 & 2.8 & PFS%


==> tables/rv_data_stub.tex <==
% bjdtdb, rv, rverr, instrument
2459456.85033 & 38136 & 35 & CHIRON \\
2459463.80033 & 38017 & 61 & CHIRON \\
2459485.70333 & 38203 & 24 & CHIRON \\
2459496.66990 & 38191 & 56 & CHIRON \\
2459539.63641 & 38086 & 26 & CHIRON%

==> tables/toi2195_gaia_comp_props.tex <==
\textit{Identifiers} & & \\
Gaia DR3 ID & 4644501668809042560 & 4644501668809042688 \\
TIC ID & 24695044 & 630977959 \\
\hline
\textit{Astrometry} & & \\
Parallax (mas)\tablenotemark{a} & $5.725 \pm 0.010$ & $5.722 \pm 0.038$ \\
$\mu_{{\alpha}}$ (mas/yr)\tablenotemark{a} & $-16.224 \pm 0.012$ & $-15.625 \pm 0.048$ \\
$\mu_{{\delta}}$ (mas/yr)\tablenotemark{a} & $-55.807 \pm 0.011$ & $-54.966 \pm 0.044$ \\
RV (km/s)\tablenotemark{a} & $39.95 \pm 0.53$ & $59.4 \pm 8.2$ \\
Ang. Sep. ($"$) & -- & 3.34 \\
Proj. Sep. (AU) & -- & 590 \\
$\mathcal{{R}}_\mathrm{{chance}}$\tablenotemark{b} & -- & $3.35 \times 10^{-6}$ \\
\hline
\textit{Photometry} & & \\
$G$ (mag)\tablenotemark{a} & $11.512 \pm 0.003$ & $15.716 \pm 0.003$ \\
$G_\mathrm{BP}$ (mag)\tablenotemark{a} & $11.928 \pm 0.003$ & $16.49 \pm 0.04$ \\
$G_\mathrm{RP}$ (mag)\tablenotemark{a} & $10.934 \pm 0.004$ & $14.41 \pm 0.01$ \\
$J$ (mag)\tablenotemark{c} & $10.254 \pm 0.034$ & -- \\
$H$ (mag)\tablenotemark{c} & $9.865 \pm 0.028$ & -- \\
$K$ (mag)\tablenotemark{c} & $9.800 \pm 0.030$ & -- \\
$W1$ (mag)\tablenotemark{d} & $9.634 \pm 0.023$ & -- \\
$W2$ (mag)\tablenotemark{d} & $9.694 \pm 0.030$ & -- \\
$W3$ (mag)\tablenotemark{d} & $9.592 \pm 0.032$ & --
